Coded Caching for Multi-level Popularity and Access

To address the exponentially rising demand for wireless content, use of caching is emerging as a potential solution. It has been recently established that joint design of content delivery and storage (coded caching) can significantly improve performance over conventional caching. Coded caching is well suited to emerging heterogeneous wireless architectures which consist of a dense deployment of local-coverage wireless access points (APs) with high data rates, along with sparsely-distributed, large-coverage macro-cell base stations (BS). This enables design of coded caching-and-delivery schemes that equip APs with storage, and place content in them in a way that creates coded-multicast opportunities for combining with macro-cell broadcast to satisfy users even with different demands. Such coded-caching schemes have been shown to be order-optimal with respect to the BS transmission rate, for a system with single-level content, i.e., one where all content is uniformly popular. In this work, we consider a system with non-uniform popularity content which is divided into multiple levels, based on varying degrees of popularity. The main contribution of this work is the derivation of an order-optimal scheme which judiciously shares cache memory among files with different popularities. To show order-optimality we derive new information-theoretic lower bounds, which use a sliding-window entropy inequality, effectively creating a non-cutset bound. We also extend the ideas to when users can access multiple caches along with the broadcast. Finally we consider two extreme cases of user distribution across caches for the multi-level popularity model: a single user per cache (single-user setup) versus a large number of users per cache (multi-user setup), and demonstrate a dichotomy in the order-optimal strategies for these two extreme cases.

==> input_files/achievability.tex <==

\subsection{Multi-user setup}
\label{sec:multi-user-achievability}

In this section, we describe the strategy used to achieve the rate approximated by the expression in Theorem~\ref{thm:multi-user-achievability}.
Moreover, we will give an exact upper bound on the achieved rate.

We will proceed in two steps.
First, we will discuss the $(H,I,J)$ partition of the set of levels as first described in Section~\ref{sec:results-multiuser}. 
This will be accompanied by an explanation of the memory-sharing parameters $\alpha_i$, which indicate what fraction of memory each level gets.
Second, we analyze the \emph{individual rate} achieved by every level $i$, after allocating $\alpha_iM$ memory to it, and combine all levels to produce the total rate achieved by the scheme.

While we actually define the $(H,I,J)$ partition based on the problem parameters, \emph{and then} choose the $\alpha_i$ values accordingly, in this paragraph we will proceed in the opposite order so that we expose the intuition behind the choices.
As discussed in Section~\ref{sec:results-multiuser}, the strategy involves finding a good partition $(H,I,J)$ of the set of levels, such that levels in $H$ are given no memory, levels in $J$ are given maximal memory, and levels in $I$ share the rest.
Thus, for all levels $h\in H$, we will assign $\alpha_hM=0$.
Similarly, every level $j\in J$ will receive $\alpha_jM=N_j/d_j$, since that is the amount of memory needed to completely store level $j$ and hence to require no BC transmission (i.e., $R^\text{SL}=0$; see Theorem~\ref{thm:single-level}).
What is left is to share the remaining memory $\left(M-\sum_{j\in J}N_j/d_j\right)$ among the levels in $I$.
More popular files should get more memory, and the popularity of a level $i$ is proportional to $U_i/N_i$.
Thus, we choose to give level $i$ a memory roughly $\alpha_iM\propto N_i\cdot\sqrt{U_i/N_i}$ (hence the memory \emph{per file} is proportional to $\sqrt{U_i/N_i}$).%
\footnote{The square root comes from minimizing an inverse function of $\alpha_i$.}

Intuitively, we want to choose $H$, $I$, and $J$ such that the above values of $\alpha_i$ are valid, i.e., $\alpha_i\in[0,1]$ for all $i$.
Based on the intuition, we get the partition described below.
\begin{definition}[$M$-feasible partition]
\label{def:m-feasible}
For any cache memory $M$, an $M$-feasible partition $(H,I,J)$ of the set of levels is a partition that satisfies:
\begin{IEEEeqnarray*}{lCl/rCcCl}
\forall h &\in& H, &
&& \tilde M &<& \frac1K \sqrt{\frac{N_h}{U_h}};\\
\forall i &\in& I, &
\frac1K \sqrt{\frac{N_i}{U_i}} &\le& \tilde M &\le& \left( \frac{1}{d_i}+\frac1K \right)\sqrt{\frac{N_i}{U_i}};\\
\forall j &\in& J, &
\left( \frac{1}{d_j} + \frac1K \right)\sqrt{\frac{N_j}{U_j}} &<& \tilde M,
\end{IEEEeqnarray*}
where $\tilde M = (M-T_J+V_I)/S_I$, and, for any subset $A$ of the levels:
\[
S_A = \sum_{i\in A} \sqrt{N_iU_i};
\quad
T_A = \sum_{i\in A} \frac{N_i}{d_i};
\quad
V_A = \sum_{i\in A} \frac{N_i}{K}.
\]
\end{definition}
We stress again that, while we used our own $\alpha_i$ values to determine $(H,I,J)$, this was done only for the intuition behind the choice.
The partition itself is defined solely based on the problem parameters, and not on our strategy.

Notice in Definition~\ref{def:m-feasible} how the different sets are largely determined by the quantity $\sqrt{N_i/U_i}$, for each level $i$.
This matches the idea that the most popular levels (i.e., those with the \emph{smallest} $N_i/U_i$) will be in $J$, while the least popular levels (those with the \emph{largest} $N_i/U_i$) will go to the set $H$.

After choosing an $M$-feasible partition, we share the memory among the levels using the following (precise) values of $\alpha_i$:
\begin{IEEEeqnarray*}{lCl"rCl}
\forall h &\in& H, & \alpha_hM &=& 0;\\
\forall i &\in& I, & \alpha_iM &=& \sqrt{N_iU_i}\cdot\tilde M - N_i/K;\\
\forall j &\in& J, & \alpha_jM &=& N_j/d_j.\IEEEyesnumber\label{eq:alpha-i}
\end{IEEEeqnarray*}
For completeness, the following proposition states the validity of this choice of memory-sharing parameters.
\begin{proposition}
The values of the memory-sharing parameters defined in \eqref{eq:alpha-i} satisfy:
\begin{enumerate}
\item $\alpha_i\ge0$ for all $i$;
\item $\sum_i\alpha_i=1$;
\item $\alpha_iM\le N_i/d_i$ for all $i$.
\end{enumerate}
Note that points 1 and 2 imply $\alpha_i\in[0,1]$.
\end{proposition}
\begin{proof}
All three results follow directly from Definition~\ref{def:m-feasible}.
\end{proof}

The structure of the solution described above allows us to efficiently compute the $\alpha_i$ values.
Indeed, Algorithm~\ref{alg:m-feasible} finds $\alpha_i$ for all levels $i$ and \emph{for all memory values $M$} in $\Theta(L^2)$ running time, where $L$ is the total number of levels.
While a detailed description and analysis of the algorithm is given in Appendix~\ref{app:multi-user-extras}, we briefly go over it in this section.
It proceeds in three main steps.
In the first step, the algorithm identifies the sequence of $(H,I,J)$ partitions that will occur as $M$ increases, using only the problem parameters.
For example, if there are two levels, there are two possible sequences, denoted below as S1 and S2:\\

\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
& & $M=0$ & & & & large $M$\\
\hline
  & $H$ & $\{1,2\}$ & $\{2\}$ & $\emptyset$ & $\emptyset$ & $\emptyset$\\
S1& $I$ & $\emptyset$ & $\{1\}$ & $\{1,2\}$ & $\{2\}$ & $\emptyset$\\
  & $J$ & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\{1\}$ & $\{1,2\}$\\
\hline
  & $H$ & $\{1,2\}$ & $\{2\}$ & $\{2\}$ & $\emptyset$ & $\emptyset$\\
S2& $I$ & $\emptyset$ & $\{1\}$ & $\emptyset$ & $\{2\}$ & $\emptyset$\\
  & $J$ & $\emptyset$ & $\emptyset$ & $\{1\}$ & $\{1\}$ & $\{1,2\}$\\
\hline
\end{tabular}
~\\

Notice that the $M$-feasible partition is the same throughout an entire interval of values for $M$.
In fact, there are only $2L$ non-trivial intervals: each interval is distinguished from the previous one by the ``promotion'' of a level from $H$ to $I$ or from $I$ to $J$.
As a result, computing only $2L$ intervals (actually, $(2L+2)$ intervals, to include the boundary cases) is enough to determine the $M$-feasible partition for \emph{all} values of $M\ge0$.

While Step 1 determines which of the above two sequences (S1 and S2) will occur, it does not determine the boundaries of the different regimes, i.e., the memory values at which the $(H,I,J)$ partition changes (except for trivial boundaries like $M=0$).
The second step computes these boundaries, using not only the problem parameters, but also the partitions themselves.

For every $M$, the corresponding $M$-feasible partition is determined by the algorithm based on the boundaries calculated in Step 2.
For example, suppose the algorithm decided that sequence S1 should be in use, and that the boundaries of $(H,I,J)=(\emptyset,\{1,2\},\emptyset)$ are some values $m_1$ and $m_2$.
Then, any $M\in[m_1,m_2]$ has $(\emptyset,\{1,2\},\emptyset)$ as its $M$-feasible partition.

\begin{algorithm}
\caption{An algorithm that constructs an $M$-feasible partition for all $M$.}
\label{alg:m-feasible}
\begin{algorithmic}[1]
\Require Number of caches $K$ and parameters $\{N_i,U_i,d_i\}_i$ for $i=1,\ldots,L$.
\Ensure An $M$-feasible partition for all $M$.

\ForAll{$i\in\{1,\ldots,L\}$}
  \State $\tilde m_i \gets (1/K)\sqrt{N_i/U_i}$
  \State $\tilde M_i \gets (1/d_i+1/K)\sqrt{N_i/U_i}$
\EndFor
\State $(x_1,\ldots,x_{2L}) \gets \mathrm{sort}(\tilde m_1,\ldots,\tilde m_L,\tilde M_1,\ldots,\tilde M_L)$.
%\Comment Sort $(\tilde m_i,\tilde M_i)$ in ascending order, and label the resulting sequence as $(x_1,\ldots,x_{2L})$.
\State

\State \emph{Step 1: Determine $(H,I,J)$ for each interval $(x_t,x_{t+1})$.}
\State Set $H_0\gets\{1,\ldots,L\}$, $I_0\gets\emptyset$, $J_0\gets\emptyset$.
\For{$t\in\{1,\ldots,2L\}$}
  \If{$x_t=\tilde m_i$ for some $i$}
    \State \emph{Promote level $i$ from $H$ to $I$}
    \State $H_t \gets H_{t-1} \setminus \{i\}$
	\State $I_t \gets I_{t-1} \cup \{i\}$
	\State $J_t \gets J_{t-1}$
  \ElsIf{$x_t=\tilde M_i$ for some $i$}
    \State \emph{Promote level $i$ from $I$ to $J$}
    \State $H_t \gets H_{t-1}$
	\State $I_t \gets I_{t-1} \setminus \{i\}$
	\State $J_t \gets J_{t-1} \cup \{i\}$
  \EndIf
\EndFor
\State

\State \emph{Step 2: Compute the limits of the intervals as $[Y_t,Y_{t+1})$.}
\ForAll{$t\in\{1,\ldots,2L\}$}
  \State $Y_t \gets x_t \cdot S_{I_t} + T_{J_t} - V_{I_t}$
\EndFor
\State $Y_{2L+1}\gets\infty$ \Comment For convenience
\State

\State \emph{Step 3: Determine the $M$-feasible partition for all $M$.}
\ForAll{$t\in\{1,\ldots,2L\}$}
  \State Set $(H_t,I_t,J_t)$ as the $M$-feasible partition of \emph{all} $M\in[Y_t,Y_{t+1})$
\EndFor
\end{algorithmic}
\end{algorithm}


The following lemma presents two important properties of $M$-feasible partitions.
It will be proved in Appendix~\ref{app:multi-user-extras}.
\begin{lemma}
\label{lemma:m-feasible-existence}
For any cache memory $M$, an $M$-feasible partition $(H,I,J)$ always exists.
Furthermore, the set $I$ is never empty as long as $M\le\sum_iN_i/d_i$, i.e., as long as individual caches do not have enough memory to store everything.
\end{lemma}

To properly analyze the achievable rate, we need to look more closely at the set $I$.
In the single-level, single-access scenario in \cite{maddah-ali2012,maddah-ali2013}, three regimes were identified, and they were analyzed separately.
Generalizing to the single-level, multi-access case, these regimes are: when $M<N/K$, when $M>cN/d$ for some constant $c\in(0,1)$, and the intermediate case.
We identify three similar regimes for each level in $i$.
Formally, define:
\begin{IEEEeqnarray*}{rCl}
I_0 &=& \left\{ i\in I : \tilde M < \frac2K\sqrt{\frac{N_i}{U_i}} \right\};\\
I_1 &=& \left\{ i\in I : \tilde M > \left(\frac{\beta}{d_i}+\frac1K\right)\sqrt{\frac{N_i}{U_i}} \right\};\\
I'  &=& I\setminus(I_0\cup I_1),
\IEEEyesnumber\label{eq:refined-partition}
\end{IEEEeqnarray*}
By choosing the $\alpha_i$ values in \eqref{eq:alpha-i}, these definitions are equivalent to: $I_0$ is the set of levels $i$ such that $\alpha_iM<N_i/K$; $I_1$ is such that $\alpha_iM>\beta N_i/d_i$ for all $i\in I_1$, where $\beta$ is the level-separation factor as defined in Regularity Condition \eqref{eq:mu-reg2}; and $I'$ consists of the remaining levels.

When $K\ge D/\beta$, then $I_0$, $I'$, and $I_1$ are mutually exclusive and form a partition of $I$.
For convenience, we call the resulting partition $(H,I_0,I',I_1,J)$ a \emph{refined $M$-feasible partition}.%
\footnote{The fact that this is a partition is important for the case $K\ge D/\beta$.
In the opposite case, this does not necessarily hold but it will not matter anyway.}

What follows is an important statement regarding the set~$I_1$.
\begin{proposition}[Size of $I_1$]
\label{prop:i1-size}
In any refined $M$-feasible partition $(H,I_0,I',I_1,J)$ as defined in Definition~\ref{def:m-feasible} and \eqref{eq:refined-partition}, the set $I_1$ contains at most one element.
\end{proposition}
\begin{proof}
Suppose that there exist two level $i,j\in I_1$ (and possibly others).
We will show that this violates regularity condition \eqref{eq:mu-reg2}.

Suppose without loss of generality that $i$ is more popular than $j$.
Since $i,j\in I_1$, then, by Definition~\ref{def:m-feasible} and \eqref{eq:refined-partition}:
\[
\left( \frac{\beta}{d_j}+\frac1K \right)\sqrt{\frac{N_j}{U_j}}
< M
\le \left( \frac{1}{d_i} + \frac1K \right)\sqrt{\frac{N_i}{U_i}}.
\]
However, this means:
\[
\sqrt{\frac{U_i/N_i}{U_j/N_j}}
< \frac{1/d_i+1/K}{\beta/d_j+1/K}
< \frac{d_j}{\beta d_i}
\le \frac{D}{\beta},
\]
which contradicts regularity condition \eqref{eq:mu-reg2}.
\end{proof}

Using the definition of a refined $M$-feasible partition, and the values of $\{\alpha_i\}_i$, we give upper bounds on the rates achieved individually for each level.
\begin{lemma}
\label{lemma:multi-user-achievability}
Given a refined $M$-feasible partition $(H,I_0,I',I_1,J)$, the individual rates of the levels are upper-bounded by:
\begin{IEEEeqnarray*}{lCl"rCl}
\forall h &\in& H, & R_h(M) &=& KU_h;\\
\forall i &\in& I_0\cup I', & R_i(M) &\le& \frac{2S_I\sqrt{N_iU_i}}{M-T_J+V_I};\\
\forall i_1 &\in& I_1, &
R_{i_1}(M) &\le& \frac1\beta d_{i_1}U_{i_1}\left( 1 - \frac{M-T_J}{N_{i_1}/d_{i_1}} \right)\\
&& & && {}+ \frac1\beta d_{i_1}U_{i_1}\frac{S_{I_0}+S_{I'}}{\sqrt{N_{i_1}U_{i_1}}};\\
\forall j &\in& J, & R_j(M) &=& 0.
\end{IEEEeqnarray*}
The total achieved rate is then:
\(
R(M) = \sum_{i=1}^L R_i(M).
\)
\end{lemma}
We relegate the proof of Lemma~\ref{lemma:multi-user-achievability} to Appendix~\ref{app:multi-user-extras}.
What follows is a brief explanation of the individual rates.
\begin{itemize}
\item
Since levels $h\in H$ get no memory, no information about their files can be stored in the caches.
Hence, the server will have to transmit a complete copy of every file requested by the $KU_h$ users in level $h$.
Therefore, $R_h(M)=KU_h$ in the worst case.

\item
Since levels $j\in J$ get maximal memory, any file requested from $j$ can be fully recovered using the caches.
Thus there is no need for the server to send anything for $j$, and hence $R_j(M)=0$.

\item
Finally, the levels $i\in I$ get enough of the remaining memory $M-T_J$ so that they behave as in Theorem~\ref{thm:single-level}.
However, since $\alpha_iM\approx\sqrt{N_iU_i}/S_I \cdot (M-T_J)$, we get a rate of:
\[
R_i(M)
\approx \frac{N_iU_i}{\alpha_iM} - d_iU_i
\approx \frac{S_I\sqrt{N_iU_i}}{M-T_J} - d_iU_i.
\]
Notice how $R_i(M)$ is inversely proportional to the memory remaining after storing $J$.
This behavior is captured in the expressions for $I_0\cup I'$.
However, for the levels in $i_1\in I_1$, which get almost, but not quite, maximal memory, the individual rate $R_{i_1}(M)$ behaves more closely to a linear function of the memory.

\end{itemize}




\subsection{Single-user setup}
\label{sec:single-user-achievability}

Recall from Section~\ref{sec:single-user-results} how the memory is divided among the sets $H'$ and $I'$, defined in \eqref{eq:G-partition}: all of the available memory is given to levels in $I'$, which is treated as one super-level.
As a result, all requests for files from $H'$ must be handled by complete file transmissions from the BS.
Since there are $\sum_{h\in H'}K_h$ users making such requests, the result is the same amount of transmissions.

For the set $I'$, now considered as one super-level, we use the single-level strategy from \cite{maddah-ali2013}.
Although only a subset of the caches is active in our setup, the same strategy still applies.
Indeed, the placement in \cite{maddah-ali2013} is a random sampling of the files in all the caches; we do the same placement in this case.
In the delivery phase, we now know the caches to which the users of $I'$ connected.
We perform a delivery as in \cite{maddah-ali2013}, assuming that only these caches were ever present in the system.

For illustration, suppose that there were $K=4$ caches.
Furthermore, assume the partition $(H',I')$ was performed such that $3$ users will request files from the set of levels $I'$.
In the placement phase, we store a random sample of the files in $I'$ in each of the four caches.
In the delivery phase, suppose the three users requesting files from $I'$ connect to caches $1$, $2$, and $4$.
In this case, the BS will send a complete file transmission for user $3$ (since he requests a file from $H'$), and will treat users $1$, $2$, and $4$ as though they were part of a single-level caching system with only three caches.

The rate required for $I'$ can be directly derived from Lemma~\ref{lemma:single-level}, using $\sum_{i\in I'} K_i$ caches, $\sum_{i\in I'} N_i$ files, and $1$ user per cache.
In addition, we have, from \eqref{eq:G-partition}, that $M\ge N_i/K_i$ for all $i\in I'$.
This implies
\(
M \ge (\sum_{i\in I'}N_i)/(\sum_{i\in I'}K_i),
\)
and hence the rate for $I'$ is:
\[
R_{I'} = \max\left\{  \frac{\sum_{i\in I'}N_i}{M}-1 \,,\, 0 \right\}.
\]
The maximization with zero is needed because it is possible to have $M>\sum_{i\in I'}N_i$.

It will be helpful for the later analysis to refine the partition $(H',I')$ as follows.
\begin{definition}
\label{def:G-partition}
Define the following partition $(G,H,I,J)$ of the set of levels:
\begin{IEEEeqnarray*}{rCl}
G &=& \left\{ g : M < N_g/K_g \text{ and } K_g\le5 \text{ and } M \le N_g/6 \right\};\\
H &=& \left\{ h : M < N_h/K_h \text{ and } K_h\ge6 \right\};\\
I &=& \left\{ i : N_i/K_i \le M \le N_i/6 \right\};\\
J &=& \left\{ j : M > N_j/6 \right\}.
\end{IEEEeqnarray*}
\end{definition}

We rewrite the achievable rate in terms of this new partition:
\begin{equation}
\label{eq:single-user-achievable-rate}
R(M)
\le 5\cdot|G|
+ \sum_{h\in H} K_h
+ \frac{\sum_{i\in I}N_i}{M}
+ \left[ \frac{\sum_{j\in J}N_j}{M} - 1 \right]^+,
\end{equation}
where $[x]^+=\max\{x,0\}$, and keeping in mind that $K_g\le5$ for $g\in G$.
If we define $N_J=\sum_{j\in J}N_j$, we can upper-bound the last term by:
\begin{equation}
\label{eq:su-ub-J}
\left[ \frac{N_J}{M} - 1 \right]^+
\le
\begin{cases}
N_J/M & \text{if $M<N_J/6$;}\\
6\left( 1 - M/N_J \right) & \text{if $N_J/6\le M < N_J$;}\\
0 & \text{if $M\ge N_J$.}
\end{cases}
\end{equation}
Effectively, the set $J$ now behaves as a unit.

Much of what defines the above partition hinges on the following question: What happens if we know the user profile \emph{a priori}?
If we do, we could imagine a strategy of total separation of the levels: every level $i$ is treated as a single-level system with $K_i$ caches and users, and $N_i$ files.
Each level can thus get the entirety of the memory of their specific $K_i$ caches.
Using Lemma~\ref{lemma:single-level}, we can calculate the total rate for this hypothetical situation as:
\[
R'(M)
= \sum_{i=1}^L
\min\left\{ K_i, \frac{N_i}{M} \right\} \left( 1 - \frac{M}{N_i} \right)^+,
\]
which can be approximated by:
\[
R'(M)
\le 5\cdot|G| + \sum_{h\in H} K_h + \sum_{i\in I} \frac{N_i}{M}
+ 6\sum_{j\in J}\left( 1-\frac{M}{N_j} \right)^+.
\]
Interestingly, the $G$, $H$, and $I$ terms in this rate expression are exactly the same as those in \eqref{eq:single-user-achievable-rate}.
Therefore, except for levels $j\in J$ where $M>N_j/6$, our scheme would not benefit from prior knowledge of the user profile.
However, the set $J$ is in general limited by the lack of this knowledge.
Indeed, if $M>N_j$ for all $j\in J$ but $M<N_J=\sum_{j\in J} N_j$, then it is possible to store any level in every cache, but it is not possible to store all levels in all caches.
Thus knowing which level is at which cache can bring the rate down to zero.

Finally, $G$ and $H$, which are both subsets of $H'$ (though not necessarily a partition; the definition of $J$ allows some of its levels to be in $H'$ too) were separated because levels behave differently when their number of caches is very small.
Specifically, a level in $H$ can transition into $I$ as the memory increases, but a level in $G$ immediately jumps to $J$ since $N_g/K_g>N_g/6$.



==> input_files/lower-bounds.tex <==

\subsection{Multi-user setup: outer bounds}

In the single-level setup introduced in \cite{maddah-ali2012}, cut-set lower bounds on the optimal rate were sufficient for proving order-optimality of the scheme.
The idea was to choose cuts that include a certain number of caches $s$, as well as enough broadcast messages to decode almost all files when combined with the $s$ caches.
The choice of $s$ depended most importantly on the size of the memory $M$.
For example, for very large $M$, the bounds would reflect the fact that a single cache should contain enough information so that it need only be combined with a small broadcast message to decode one file.
In contrast, for small $M$, the bounds would instead show that a large broadcast message is needed to serve all $s$ users.

In our multi-level situation, the goal of our lower bounds is to show that different popularity levels require different amounts of memory, ranging from zero to maximal memory.
However, a single cut-set bound would force all levels to abide by the same number of caches $s$, a choice that would not reflect the plurality of memory allocation.
New lower bounds were thus required.

The lower bounds that we use allow choosing for each level $i$ the number of caches $s_i$ that corresponds to the amount of memory we expect it to get.
In essence, each level $i$ will exclusively be part of a cut-set bound with $s_i$ caches, which will give a lower bound that loosely corresponds to  the individual rate $R_i$ for this level.

The challenge is to incorporate all of these cut-set bounds together, such that the same caches appear in cut-set bounds for all levels.
This process is described next.
We start with a cut-set bound for the level with the smallest $s_i$.
Using Fano's inequality, we can derive lower bounds on its individual rate.
We then proceed to lower-bound the current quantity using a cut-set bound for the level with the next smallest $s_i$, and repeat the process.
The transition from one cut-set bound to the next can be achieved using sliding-window subset entropy inequalities \cite[Theorem~3]{Liu14}:%
\footnote{For these inequalities to work, we have to take not just one cut-set bound per level, but an averaging of $K$ similar cut-set bounds that ends up including all caches an equal number of times.}
\begin{lemma}[Sliding-window subset entropy inequality {\cite[Theorem~3]{Liu14}}]
\label{lemma:sliding-window}
Given $K$ random variables $(Y_1,\ldots,Y_K)$, we have, for every $s\in\{1,\ldots,K-1\}$:
\[
\frac1s\sum_{i=1}^K H\left(Y_i,\ldots,Y_{\langle i+s-1\rangle}\right)
\ge
\frac{1}{s+1}\sum_{i=1}^K
H\left( Y_i,\ldots,Y_{\langle i+s\rangle} \right),
\]
where we define $\langle i\rangle = i$ if $i\le K$ and $\langle i\rangle = i-K$ if $i>K$.
\end{lemma}

The resulting lower bounds, in their final form, are given in the following lemma.
\begin{lemma}
\label{lemma:multi-user-converse}
Consider the multi-level, multi-user caching setup.
Let $b\in\mathbb{N}^+$ and $t\in\{1,\ldots,K\}$.
Furthermore, for every level $i$, let $s_i\in\mathbb{N}^+$ such that $s_it\in\{d_i,\ldots,\floor{K/2}\}$.
Then, for every memory $M$, the optimal rate can be bounded from below by:
\[
R^\ast(M)
\ge \sum_{i=1}^L
\lambda_i
\cdot \min\left\{ (s_it-d_i+1)U_i \,,\,\frac{N_i}{s_ib} \right\}
- \frac tb M,
\]
where $\lambda_i$ is a constant (introduced for technical reasons) defined as: $\lambda_i=1$ if $s_it=d_i$; and $\lambda_i=\frac12$ if $s_it>d_i$.
\end{lemma}

The full proof of Lemma~\ref{lemma:multi-user-converse} is given in Appendix~\ref{app:multi-user-converse}.
However, we will here give a brief intuition behind the expression shown above.
Every term in the sum corresponds to a level $i$.
Consider a single level $i$.
Roughly, if we ignore all the other levels in the summation, and assuming $d_i=1$ for simplicity, then the inequality can be rearranged approximately as follows:
\[
s_ib R + s_it M \ge \min\left\{ s_it\cdot s_ib\cdot U_i \,,\, N_i \right\}.
\]
This expression is essentially a cut-set bound, saying that, with $s_it$ caches and $s_ib$ broadcast messages, up to $s_it\cdot s_ib\cdot U_i$ files from level $i$ can be decoded (since there are $U_i$ users per cache for this level), unless this number excedes the total number of files $N_i$.


\subsection{Multi-user setup: approximate optimality}

In order to prove order-optimality of the memory-sharing scheme, we must use Lemma~\ref{lemma:multi-user-converse} with appropriate parameters.
Our goal is to get a resulting lower bound on the optimal rate $R^\ast(M)$ such that the ratio between the achievable rate and $R^\ast(M)$---henceforth called the \emph{gap}---is minimized.
More specifically, the result we seek is a constant upper bound on the gap.

For technical reasons, several cases need to be considered for which different values are chosen for the parameters in Lemma~\ref{lemma:multi-user-converse}.
In particular, the values of choice in one case would violate the conditions imposed on them in another case.
In this section, we will illustrate the proof methodology by approximating one of these cases.
The complete and rigorous proof is given in Appendix~\ref{app:multi-user-gap}.

Recall the refined $M$-feasible partition introduced in Definition~\ref{def:m-feasible} and in \eqref{eq:refined-partition}.
As previously mentioned, this partition only depends on the problem parameters, not on the achievability strategy.
The cases of interest for the proof of order-optimality are:
\begin{itemize}
\item Case 1a: $I_1=\emptyset$ and $J\not=\emptyset$;
\item Case 1b: $I_1=\emptyset$ and $J=\emptyset$;
\item Case 2: $I_1\not=\emptyset$.
\end{itemize}
There is also a special Case 0 for when $K$ is small (specifically, $K<D/\beta$).
All the other cases assume $K$ is large.

The case that we will focus on in this section is Case 1a.
Note that $I_1=\emptyset\implies I=I_0\cup I'$.
For simplicity, we will assume that $d_i=1$ for all $i$.
Furthermore, most of the analysis will be approximate.

By Lemma~\ref{lemma:multi-user-achievability}, the achievable rate in Case 1a can be upper-bounded by:
\begin{equation}
\label{eq:approx-achievable-rate}
R(M) \le \sum_{h\in H} KU_h + \frac{2S_I^2}{M-T_J},
\end{equation}
since $S_I=\sum_{i\in I}\sqrt{N_iU_i}$ (see Definition~\ref{def:m-feasible}).
Now consider Lemma~\ref{lemma:multi-user-converse} with the following parameters:
\begin{IEEEeqnarray*}{lCl"rCl}
&& & t &=& 1;\\
\forall h&\in&H, & s_h &\approx& \frac12K;\\
\forall i&\in&I, & s_i &\approx& \frac{\sqrt{N_i/U_i}}{2\tilde M};\\
\forall j&\in&J, & s_j &=& 1;\\
&& & b &\approx& 4 \tilde M^2,
\end{IEEEeqnarray*}
where, as in Definition~\ref{def:m-feasible}, $\tilde M = (M-T_J+V_I)/S_I \approx (M-T_J)/S_I$.
The values of the $s_i$'s are very similar to those used in the single-level setup in \cite{maddah-ali2012}.
Indeed, the levels with the smallest memory ($h\in H$) are handled using cut-set bounds that consider a fraction of the total number of caches, while the levels with the largest memory ($j\in J$) are handled with bounds that consider only one cache.
Thus, the lemma lower-bounds the optimal rate by:
\begin{IEEEeqnarray*}{rCl}
R^\ast(M)
&\ge& \sum_{h\in H} \min\left\{ s_hU_h, \frac{N_h}{s_hb} \right\}
+ \sum_{i\in I} \min\left\{ s_iU_i, \frac{N_i}{s_ib} \right\}\\
&&{} + \sum_{j\in J} \min\left\{ s_jU_j, \frac{N_j}{s_jb} \right\}
- \frac{M}{b}.
\end{IEEEeqnarray*}
Substituting the values of the parameters, and utilizing the inequalities on $\tilde M$ that define the refined $M$-feasible partition, we get:
\begin{IEEEeqnarray*}{rCl}
R^\ast(M)
&\ge& \sum_{h\in H} \frac12 KU_h
+ \sum_{i\in I} \frac{\sqrt{N_iU_i}S_I}{2(M-T_J)}
+ \sum_{j\in J} \frac{N_j}{b}
- \frac{M}{b}\\
&=& \sum_{h\in H} \frac12KU_h
+ \frac{S_I^2}{2(M-T_J)}
- \frac{M-T_J}{b}\\
&=& \sum_{h\in H} \frac12KU_h
+ \frac{S_I^2}{2(M-T_J)}
- \frac{(M-T_J)S_I^2}{4(M-T_J)^2}\\
&=& \sum_{h\in H} \frac12KU_h
+ \frac{S_I^2}{4(M-T_J)}\\
&\overset{(a)}{\ge}& \frac{1}{8}\cdot R(M).
\end{IEEEeqnarray*}
The last inequality $(a)$ is due to \eqref{eq:approx-achievable-rate}.

Thus, the result is a constant multiplicative gap ($8$ in this example) between the achievable rate and the optimal rate for this regime.
The full proof in Appendix~\ref{app:multi-user-gap} derives such gaps for each one of the four regimes mentioned above (Cases 0, 1a, 1b, and 2), and finally combines them into one multiplicative gap that holds for all cases.




\subsection{Single-user setup}
\label{sec:single-user-gap}

As mentioned in Section~\ref{sec:single-user-results}, we use a cut-set bound to lower-bound the optimal rate.
The idea is to send a certain number $b$ of broadcast messages $X_1,\ldots,X_b$ that serve certain requests.
We choose these requests as follows.
For every level $i\in G\cup H\cup I$, consider a certain number $s_i\le K_i$ of caches.
These caches are distinct across levels.
For all the $b$ broadcasts, the users connected to these $s_i$ caches will altogether request $s_ib$ distinct files from level $i$ if there are that many; otherwise they request all $N_i$ files.
For the levels in the set $J$, we collectively consider some $s_J$ caches (distinct from the rest).
The users at these $s_J$ caches will use all $b$ broadcasts to decode as many files from the set $J$ as possible, up to $s_Jb$ files.
Let $n_J$ denote this number; it will be determined later.

If we let $S=\sum_{i\not\in J}s_i + s_J$ be the total number of caches considered, then, by Fano's inequality:
\begin{IEEEeqnarray*}{rCl}
bR + SM
&\ge& H\left( Z_1,\ldots,Z_S,X_1,\ldots,X_b \right)\\
&\ge& \sum_{i\not\in J} \min\left\{ s_ib,N_i \right\} + n_J\\
R^\ast(M) &\ge& \sum_{i\not\in J} s_i\left( \min\left\{ 1,\frac{N_i}{s_ib} \right\} - \frac{M}{b} \right)\\
&& {} + s_J\left( \frac{n_J}{s_Jb} - \frac{M}{b} \right)\\
&=& \sum_{i\not\in J} v_i + v_J. \IEEEyesnumber\label{eq:single-user-lower-bounds}
\end{IEEEeqnarray*}

We will analyze each of the $v_i$ and $v_J$ terms separately.
We identify two cases for which the analysis is slightly different.

The first case is when $M<1/6$.
Because of regularity condition \eqref{eq:su-reg}, this implies $M<1/6<1\le N_i/K_i$ for all levels $i$, and thus the achievable rate can be bounded by:
\begin{equation}
\label{eq:su-ub-0}
R(M) \le \sum_{i=1}^L K_i.
\end{equation}
The second case, which is more interesting, is when $M\ge1/6$.

The details of the analysis are given in Appendix~\ref{app:single-user-gap}.
We will here give a brief outline of the procedure, with approximations to avoid burying the essence of the argument under technicalities.
The idea is to lower-bound each term $v_i$ or $v_J$ to match the corresponding term in the rate expression.
Let us focus on the case $M\ge1/6$, and suppose we choose $b\approx6M\ge1$.
For simplicity, we will only look at the sets $H$ and $I$.

Consider a level $h\in H$, and let $s_h\approx K_h/6$.
Then, by the definition of $H$:
\[
\frac{N_h}{s_hb} = \frac{N_h}{K_hM} \ge 1.
\]
As a result,
\[
v_h = \frac{K_h}{6}\left( 1 - \frac{M}{6M} \right) = \frac{5}{36}\cdot K_h,
\]
which matches the corresponding achievable rate term in \eqref{eq:single-user-achievable-rate}, up to the constant $(5/36)$.

Now consider a level $i\in I$, and let $s_i\approx N_i/(6M)$.
Then,
\[
\frac{N_i}{s_ib} = \frac{N_i}{(N_i/6M)\cdot6M} = 1,
\]
and hence:
\[
v_i = \frac{N_i}{6M}\left( 1 - \frac{M}{6M} \right) = \frac{5}{36}\cdot\frac{N_i}{M}.
\]
Again, this matches the corresponding achievable rate term in \eqref{eq:single-user-achievable-rate}, up to the constant $(5/36)$.

Applying a similar procedure for every level, we get matching lower bounds (up to a constant) and thus prove Theorem~\ref{thm:single-user-gap}.





==> input_files/small-example.tex <==

%\subsection{A small, illustrative example}

\begin{figure}
\centering
\includegraphics[width=\myfigswidth]{setup2p4u.pdf}
\caption{Setup for the small example. It is assumed that $N_2\ge4$.}
\label{fig:small-example}
\end{figure}

We illustrate our problem setup with the small example shown in \figurename~\ref{fig:small-example}.
The BS holds files of $L=2$ different popularity levels: $N_1=2$ popular files $\{W^1_1,W^1_2\}$, and $N_2\ge4$ unpopular files $\{W_1^2, W_2^2, \ldots, W^2_{N_2}\}$.
Each file has a size of $F$ bits.
There are $K=2$ APs, each equipped with a cache of size $MF$ bits whose contents are denoted by $Z_1$ and $Z_2$.
There are $U = 3$ users in the system. 

The system is operated in two phases.
During the \emph{placement phase}, each cache stores content related to the files without any prior knowledge of the user requests.
Later, during the \emph{delivery phase}, the users place their requests.
Users 1 and 2 request popular files, say $W^1_{r_1}$ and $W^1_{r_2}$ respectively, and user 3 requests an unpopular file, say $W^2_{r_3}$.
Furthermore, users 1 and 2 access the cache contents of AP 1 and 2 respectively, while user 3 is required to access both APs.
In addition, all users can listen to a common BS broadcast $X^\mathbf{r}$ of size $RF$ bits, where $\mathbf{r}=(r_1,r_2,r_3)$ denotes the request vector.
Using only the accessed cache contents and the BS transmission, each user attempts to recover their requested file. 

The pair $(R, M)$ is said to be \emph{feasible} if there exists a placement scheme with normalized cache size $M$, such that, for \emph{every} request vector $\mathbf{r}$, there exists a BS broadcast transmission $X^\mathbf{r}$ of rate no greater than $R$ such that all the requests are satisfied.
For any value of the memory size $M$, denote the optimal BS transmission rate over all
possible schemes by:
\begin{equation}
\label{eq:optimal-rate}
R^\ast(M) = \inf \left\{ R : (M,R) \text{ is feasible} \right\}, 
\end{equation}
where the minimization is over \emph{all} feasible strategies. 

%
\begin{figure}
\centering
\includegraphics[width=\myfigswidth]{2p4u_region.pdf}
\caption{Optimal rate $R^\ast(M)$ for the example in \figurename~\ref{fig:small-example}.}
\label{fig:small-example-ratemem}
\end{figure}
%

For the example in \figurename~\ref{fig:small-example}, we illustrate the minimum achievable rate $R^\ast(M)$ for every value of memory size $M$ in \figurename~\ref{fig:small-example-ratemem}. 
The following theorem formalizes this result.
\begin{theorem}
\label{thm:small-example}
For the caching setup given in \figurename~\ref{fig:small-example}, the optimal rate-memory trade-off is given by:
\[
R^\ast(M)
= \max\left\{
3 - 2M,
\frac52 - M,
2 - \frac12 M,
1 - \frac{M-2}{N_2/2}
\right\}.
\]
\end{theorem}
The proof Theorem~\ref{thm:small-example} is given in Appendix~\ref{app:small-example}.
However, the next paragraph will discuss the achievability of one $(R,M)$-point to illustrate the result.

Let us consider the corresponding achievable scheme for the specific tuple $(R,M)=(\frac32,1)$.
Recall that a memory of $M=1$ means that each cache can hold up to the size of one file.
We split each of the popular files $W^1_1$ and $W^1_2$ into two halves: $W^1_1=(W^1_{1a},W^1_{1b})$ and $W^1_2=(W^1_{2a},W^1_{2b})$. 
Let the cache contents be $Z_1 = (W^1_{1a}, W^1_{2a})$ and $Z_2 = (W^1_{1b}, W^1_{2b})$, thus satisfying the memory size constraint.
When the user requests are revealed, the BS sends a broadcast of two parts: $X^\mathbf{r}=(X_1^\mathbf{r},X_2^\mathbf{r})$.
The first part, $X_1^\mathbf{r}=W^2_{r_3}$, satisfies the request of user 3 for an unpopular file.
The second part, $X_2^\mathbf{r}=W^1_{r_1b}\oplus W^1_{r_2a}$, along with the accessed AP cache content, enables both users 1 and 2 to recover their requested files.
Additionally, we use an information-theoretic bound to prove the optimality of the above described scheme for $M = 1$. 

While, for this small example, we were able to derive the optimal scheme for every value of $M$, it is in general difficult to extend this method to networks with a larger number of caches, users, or file classes.
Hence, we will instead focus on identifying \emph{order-optimal} schemes, for which the achievable rate $R(M)$ is within a constant multiplicative factor of the optimal rate $R^*(M)$, i.e., $R(M) / R^\ast(M) \leq c$, where $c$ is independent of the problem parameters.



\begin{comment}

In the next section, we illustrate our achievability scheme on a specific example with four levels.
Later, our main result in Theorem~\ref{thm:main} proves the order-optimality of the general scheme.


\subsection{Example: achievability scheme}

Suppose the BS holds a total of $N = 62{,}100$ files of size $F$ bits each, divided into $L=4$ levels with $N_1 = 900$, $N_2 = 2700$, $N_3 = 10{,}500$, and $N_4 = 48{,}000$ files in different levels.
The four  levels represent different file popularities, with level 1 consisting of the most popular files and level 4 including the least popular files.
Suppose also that there are $K=25$ APs, and $U_1=25$, $U_2=16$, $U_3=7$, and $U_4=1$ users accessing each AP, requesting files of levels $1$, $2$, $3$, and $4$, respectively.
Finally, suppose that each AP has a cache of size $MF=3600F$ bits.

Given such a setup, we want to identify what should be stored in each AP cache and how the requested files should be delivered, so that the associated BS transmission rate is minimized. 
One natural strategy would be to allocate the entire memory of each cache to store as many popular files as possible.
Since $M=N_1+N_2$ in this example, this would mean storing all the files of levels $1$ and $2$ in each of the caches.
As a result, the users requesting files from levels $1$ or $2$ can satisfy their demands by only accessing the corresponding APs.
On the other hand, the $K(U_3+U_4)=200$ users requesting files of levels 3 and 4 have to rely solely on the BS broadcast.
Since all these requests can be for different files, the  peak BS transmission size is $RF=200F$ bits.

Let us now consider an alternate scheme.
We partition the set of file levels $\{1,2,3,4\}$ into three subsets: $H$, $I$, and $J$.
Each level $i$ is allotted a portion $\alpha_iM$ of each cache memory, $\alpha_i\in[0,1]$, depending on the set to which it belongs.
Levels in $H$ are assigned no cache memory ($\alpha_iM=0$), and thus the corresponding requests are solely served by the BS transmission.
Each level in the set $J$ is assigned enough memory so that every cache can hold all its constituent files, i.e., $\alpha_iM=N_i$.
Finally, the remaining memory is shared among the levels in set $I$, so as to minimize the resulting BS transmission rate.
Note that the values of the $\alpha_i$ parameters depend on the cache memory $M$.
The assignment of the levels to the subsets $H$, $I$, and $J$ is done such that the levels assigned to $J$ are more popular than the levels in $I$, which in turn dominate the levels in $H$.
This ensures that more popular content is given a relatively larger portion of the cache.

For our setup with $M = 3600$, let $H=\{4\}$, $I=\{3,2\}$, $J=\{1\}$, and set $\alpha_1=N_1/M=0.25$, $\alpha_2=0.35$, $\alpha_3=0.4$, and $\alpha_4=0$. Next, we treat each level $i$ as a separate sub-system with $N_i$ files, $K$ APs, $U_i$ users per AP, and $\alpha_iM$ cache memory.
Each of these sub-systems has single-level content, and, as mentioned earlier, such a setup was studied in \cite{maddah-ali2012}.
Using the coded caching scheme proposed in \cite{maddah-ali2012} for each of these sub-systems, the total required BS transmission rate is given by  
%
$
\sum_{i = 1}^{L} r_c\left(\alpha_i M / N_i, K, U_i \right), 
$
%
where $r_c(M / N, K, U)$ denotes the achievable rate in a single-level system with $N$ files, $K$ APs, each with memory size $M$, and $U$ users accessing every cache.
Evaluating the rate expression for our choice of $\alpha_i$'s, we get a peak BS transmission size of approximately $76.4F$, which is an improvement by a factor of about $2.62$ over the first scheme.
The scheme illustrated for the above example can be extended to the  general setup by carefully choosing the subsets $(H,I,J)$ and the memory-sharing parameters $\alpha_i$'s.
We briefly discuss this in Section~\ref{Sec:AchievableRate} and give details in \cite{isit2014_extended}. 
%

Illustrated by the examples above, our general problem statement is as follows.
Consider a caching system with a BS holding $L$ levels of content, consisting of $N_1, \ldots, N_L$ files.
There are $K$ APs, each equipped with a cache of normalized size $M$, and $U_1, \ldots, U_L$ users accessing each AP with requests for a file from level $1$, \ldots, level $L$, respectively.
Given such a setup, we want to characterize the minimum achievable BS transmission rate $R^*(M)$, for any cache memory size $M$.  


\end{comment}







